Evaluation of Generalizability of Neural Program Analyzers under Semantic-Preserving Transformations

The abundance of publicly available source code repositories, in conjunction with the advances in neural networks, has enabled data-driven approaches to program analysis. These approaches, called neural program analyzers, use neural networks to extract patterns in the programs for tasks ranging from development productivity to program reasoning. Despite the growing popularity of neural program analyzers, the extent to which their results are generalizable is unknown. In this paper, we perform a large-scale evaluation of the generalizability of two popular neural program analyzers using seven semantically-equivalent transformations of programs. Our results caution that in many cases the neural program analyzers fail to generalize well, sometimes to programs with negligible textual differences. The results provide the initial stepping stones for quantifying robustness in neural program analyzers.

==> evaluation-approach/seeds.tex <==
\subsection{Seeds}
\iTODO{relation between loss and confidence}
\iTODO{More rewarding: fooling high-confidence}
\iTODO{Low-hanging: high loss can be a target}

==> motivating-example/boolean-exchange.tex <==
%\subsubsection{Boolean Exchange}

\begin{figure*}
\caption*{Boolean Exchange: java-small/test/hadoop/BlockPoolManager.java}
\noindent \begin{minipage}{.5\textwidth}
\begin{lstlisting}[basicstyle=\fontsize{9}{11}\selectfont, title= Prediction before transformation: \textbf{\textcolor{blue}{remove}}]
synchronized void remove(BPOfferService t) {
    [...]
    boolean removed = <@\textbf{\textcolor{blue}{false}}@>;
    for ([...]; it.hasNext() && <@\textbf{\textcolor{blue}{!removed}}@>; ) {
        BPOfferService bpos = it.next();
        if (bpos == t) {
            it.remove();
            LOG.info("Removed " + bpos);
            removed = <@\textbf{\textcolor{blue}{true}}@>;
        }
    }
    if (<@\textbf{\textcolor{blue}{!removed}}@>) {
        LOG.warn([...]);
    }
}
\end{lstlisting}
\end{minipage}%
\begin{minipage}{.5\textwidth}
\begin{lstlisting}[basicstyle=\fontsize{9}{11}\selectfont, title= Prediction after transformation: \textbf{\textcolor{red}{decode}}]
synchronized void remove(BPOfferService t) {
    [...]
    boolean removed = <@\textbf{\textcolor{red}{true}}@>;
    for ([...]; it.hasNext() && <@\textbf{\textcolor{red}{removed}}@>; ) {
        BPOfferService bpos = it.next();
        if (bpos == t) {
            it.remove();
            LOG.info("Removed " + bpos);
            removed = <@\textbf{\textcolor{red}{false}}@>;
        }
    }
    if (<@\textbf{\textcolor{red}{removed}}@>) {
        LOG.warn([...]);
    }
}
\end{lstlisting}
\end{minipage}
\end{figure*}


==> motivating-example/loop-exchange.tex <==
%\subsubsection{Loop Exchange}

\begin{figure*}
\caption*{Loop Exchange: java-small/test/hadoop/BaileyBorweinPlouffe.java}
\noindent \begin{minipage}{.5\textwidth}
\begin{lstlisting}[basicstyle=\fontsize{9}{11}\selectfont, title= Prediction before transformation: \textbf{\textcolor{blue}{sum}}]
private static double sum(final long j, final long d) {
    [...]
    <@\textbf{\textcolor{blue}{for (; ; k++)}}@> {
        final long n = (k << 3) | j;
        final long shift = (k - d) << 2;
        if (ACCURACY_BIT <= shift || 1L << (ACCURACY_BIT - shift) < n) {
            return s;
        }
        s += 1.0 / (n << shift);
        if (s >= 1)
            s--;
        <@$\newline$@>
    }
}
\end{lstlisting}
\end{minipage}%
\begin{minipage}{.5\textwidth}
\begin{lstlisting}[basicstyle=\fontsize{9}{11}\selectfont, title= Prediction after transformation: \textbf{\textcolor{red}{position}}]
private static double sum(final long j, final long d) {
    [...]
    <@\textbf{\textcolor{red}{while (true)}}@> {
        final long n = (k << 3) | j;
        final long shift = (k - d) << 2;
        if (ACCURACY_BIT <= shift || 1L << (ACCURACY_BIT - shift) < n) {
            return s;
        }
        s += 1.0 / (n << shift);
        if (s >= 1)
            s--;
        <@\textbf{\textcolor{red}{k++;}}@>
    }
}
\end{lstlisting}
\end{minipage}
\end{figure*}



==> motivating-example/permute-stmt.tex <==
%\subsubsection{Permute Statement}

\begin{figure*}
\caption*{Permute Statement: java-small/test/hadoop/TestOutOfOrderWrite.java}
\noindent \begin{minipage}{.5\textwidth}
\begin{lstlisting}[basicstyle=\fontsize{7}{11}\selectfont, title= Prediction before transformation: \textbf{\textcolor{blue}{message|received}}]
public void messageReceived(ChannelHandlerContext ctx, MessageEvent e) {
    // Get handle from create response
    ChannelBuffer buf = (ChannelBuffer) e.getMessage();
    XDR rsp = new XDR(buf.array());
    if (rsp.getBytes().length == 0) {
        LOG.info("rsp length is zero, why?");
        return;
    }
    LOG.info("rsp length=" + rsp.getBytes().length);
    RpcReply reply = RpcReply.read(rsp);
    int xid = reply.getXid();
    // Only process the create response
    if (xid != 0x8000004c) {
        return;
    }
    int status = rsp.readInt();
    if (status != Nfs3Status.NFS3_OK) {
        LOG.error("Create failed, status =" + status);
        return;
    }
    <@\textbf{\textcolor{blue}{LOG.info("Create succeeded");}}@>
    // value follow
    rsp.readBoolean();
    <@\textbf{\textcolor{blue}{handle = new FileHandle();}}@>
    handle.deserialize(rsp);
    channel = e.getChannel();
}
\end{lstlisting}
\end{minipage}%
\begin{minipage}{.5\textwidth}
\begin{lstlisting}[basicstyle=\fontsize{7}{11}\selectfont, title= Prediction after transformation: \textbf{\textcolor{red}{read}}]
public void messageReceived(ChannelHandlerContext ctx, MessageEvent e) {
    // Get handle from create response
    ChannelBuffer buf = (ChannelBuffer) e.getMessage();
    XDR rsp = new XDR(buf.array());
    if (rsp.getBytes().length == 0) {
        LOG.info("rsp length is zero, why?");
        return;
    }
    LOG.info("rsp length=" + rsp.getBytes().length);
    RpcReply reply = RpcReply.read(rsp);
    int xid = reply.getXid();
    // Only process the create response
    if (xid != 0x8000004c) {
        return;
    }
    int status = rsp.readInt();
    if (status != Nfs3Status.NFS3_OK) {
        LOG.error("Create failed, status =" + status);
        return;
    }
    <@\textbf{\textcolor{red}{handle = new FileHandle();}}@>
    // value follow
    rsp.readBoolean();
    <@\textbf{\textcolor{red}{ LOG.info("Create succeeded");}}@>
    handle.deserialize(rsp);
    channel = e.getChannel();
}
\end{lstlisting}
\end{minipage}
\end{figure*}



==> motivating-example/switch-to-if.tex <==
%\subsubsection{Switch to If}

\begin{figure*}
\caption*{Switch to If: java-small/test/hadoop/TestValueIterReset.java}
\noindent \begin{minipage}{.5\textwidth}
\begin{lstlisting}[basicstyle=\fontsize{8}{11}\selectfont, title= Prediction before transformation: \textbf{\textcolor{blue}{reduce}}]
public void reduce(IntWritable key, Iterable<IntWritable> values, Context context) throws IOException, InterruptedException {
    int errors = 0;
    MarkableIterator<IntWritable> mitr = new MarkableIterator<IntWritable>(values.iterator());
    <@\textbf{\textcolor{blue}{switch}}@>(key.get()) {
        <@\textbf{\textcolor{blue}{case 0}}@>:
            errors += test0(key, mitr);
            break;
        <@\textbf{\textcolor{blue}{case 1}}@>:
            errors += test1(key, mitr);
            break;
        <@\textbf{\textcolor{blue}{case 2}}@>:
            errors += test2(key, mitr);
            break;
        <@\textbf{\textcolor{blue}{case 3}}@>:
            errors += test3(key, mitr);
            break;
        <@\textbf{\textcolor{blue}{default}}@>:
            break;
    }
    context.write(key, new IntWritable(errors));
}
\end{lstlisting}
\end{minipage}%
\begin{minipage}{.5\textwidth}
\begin{lstlisting}[basicstyle=\fontsize{8}{11}\selectfont, title= Prediction after transformation: \textbf{\textcolor{red}{put}}]
public void reduce(IntWritable key, Iterable<IntWritable> values, Context context) throws IOException, InterruptedException {
    int errors = 0;
    MarkableIterator<IntWritable> mitr = new MarkableIterator<IntWritable>(values.iterator());
    <@$\newline$@>
    <@\textbf{\textcolor{red}{if}}@> (key.get() == 0) {
        errors += test0(key, mitr);
        <@$\newline$@>
    } <@\textbf{\textcolor{red}{else if}}@> (key.get() == 1) {
        errors += test1(key, mitr);
        <@$\newline$@>
    } <@\textbf{\textcolor{red}{else if}}@> (key.get() == 2) {
        errors += test2(key, mitr);
        <@$\newline$@>
    } <@\textbf{\textcolor{red}{else if}}@> (key.get() == 3) {
        errors += test3(key, mitr);
        <@$\newline$@>
    } <@\textbf{\textcolor{red}{else}}@> {
        <@$\newline$@>
    }
    context.write(key, new IntWritable(errors));
}
\end{lstlisting}
\end{minipage}
\end{figure*}


==> motivating-example/trycatch-insertion.tex <==
%\subsubsection{Try Catch Insertion}

\begin{figure*}
\caption*{Try Catch Insertion: java-small/test/hadoop/DominantResourceFairnessPolicy.java}
\noindent \begin{minipage}{.5\textwidth}
\begin{lstlisting}[basicstyle=\fontsize{7.5}{11}\selectfont, title= Prediction before transformation: \textbf{\textcolor{blue}{compare}}]
public int compare(Schedulable s1, Schedulable s2) {
    [...]
    boolean s1Needy = sharesOfMinShare1.getWeight(resourceOrder1[0]) < 1.0f;
    boolean s2Needy = sharesOfMinShare2.getWeight(resourceOrder2[0]) < 1.0f;
    int res = 0;
    <@$\newline$@>
    if (!s2Needy && !s1Needy) {
        res = compareShares(sharesOfCluster1, sharesOfCluster2, resourceOrder1, resourceOrder2);
    } else if (s1Needy && !s2Needy) {
        res = -1;
    } else if (s2Needy && !s1Needy) {
        res = 1;
    } else {
        // both are needy below min share
        res = compareShares(sharesOfMinShare1, sharesOfMinShare2, resourceOrder1, resourceOrder2);
    }
    <@$\newline$@>
    <@$\newline$@>
    <@$\newline$@>
    [...]
    return res;
}
\end{lstlisting}
\end{minipage}%
\begin{minipage}{.5\textwidth}
\begin{lstlisting}[basicstyle=\fontsize{7.5}{11}\selectfont, title= Prediction after transformation: \textbf{\textcolor{red}{add}}]
public int compare(Schedulable s1, Schedulable s2) {
    [...]
    boolean s1Needy = sharesOfMinShare1.getWeight(resourceOrder1[0]) < 1.0f;
    boolean s2Needy = sharesOfMinShare2.getWeight(resourceOrder2[0]) < 1.0f;
    int res = 0;
    <@\textbf{\textcolor{red}{try \{}}@>
        if (!s2Needy && !s1Needy) {
            res = compareShares(sharesOfCluster1, sharesOfCluster2, resourceOrder1, resourceOrder2);
        } else if (s1Needy && !s2Needy) {
            res = -1;
        } else if (s2Needy && !s1Needy) {
            res = 1;
        } else {
            // both are needy below min share
            res = compareShares(sharesOfMinShare1, sharesOfMinShare2, resourceOrder1, resourceOrder2);
        }
    <@\textbf{\textcolor{red}{\} catch (Exception ex) \{}}@>
        <@\textbf{\textcolor{red}{ex.printStackTrace();}}@>
    <@\textbf{\textcolor{red}{\}}}@>
    [...]
    return res;
}
\end{lstlisting}
\end{minipage}
\end{figure*}

==> motivating-example/unreachable-stmt-insertion.tex <==
%\subsubsection{Unreachable Statement Insertion}

\begin{figure*}
\caption*{Unreachable Statement Insertion: java-small/test/hadoop/BlockCompressorStream.java}
\noindent \begin{minipage}{.5\textwidth}
\begin{lstlisting}[title= Prediction before transformation: \textbf{\textcolor{blue}{compress}}]
protected void compress() throws IOException {
    int len = compressor.compress(buffer, 0, buffer.length);
    if (len > 0) {
        // Write out the compressed chunk
        rawWriteInt(len);
        out.write(buffer, 0, len);
    }
}
<@$\newline$@>
<@$\newline$@>
<@$\newline$@>
\end{lstlisting}
\end{minipage}%
\begin{minipage}{.5\textwidth}
\begin{lstlisting}[title= Prediction after transformation: \textbf{\textcolor{red}{read}}]
protected void compress() throws IOException {
    int len = compressor.compress(buffer, 0, buffer.length);
    <@\textbf{\textcolor{red}{if (false) \{}}@>
        <@\textbf{\textcolor{red}{System.out.println("an unreachable statement");}}@>
    <@\textbf{\textcolor{red}{\}}}@>
    if (len > 0) {
        // Write out the compressed chunk
        rawWriteInt(len);
        out.write(buffer, 0, len);
    }
}
\end{lstlisting}
\end{minipage}
\end{figure*}

==> motivating-example/unused-stmt-insertion.tex <==
%\subsubsection{Unused Statement Insertion}

\begin{figure*}
\caption*{Unused Statement Insertion: java-small/test/hadoop/StreamPumper.java}
\noindent \begin{minipage}{.5\textwidth}
\begin{lstlisting}[basicstyle=\fontsize{8.5}{11}\selectfont, title= Prediction before transformation: \textbf{\textcolor{blue}{start}}]
void start() {
    assert !started;
    thread.start();
    started = true;
}
<@$\newline$@>
\end{lstlisting}
\end{minipage}%
\begin{minipage}{.5\textwidth}
\begin{lstlisting}[basicstyle=\fontsize{8.5}{11}\selectfont, title= Prediction after transformation: \textbf{\textcolor{red}{stop}}]
void start() {
    assert !started;
    thread.start();
    <@\textbf{\textcolor{red}{String dummy\_timestamp = "2019-10-28 02:52:10.782";}}@>
    started = true;
}
\end{lstlisting}
\end{minipage}
\end{figure*}

==> recycle-bin.tex <==
\begin{comment}
Table~\ref{tab:data} summarizes the \npas and the datasets that we use in the experiment.

    \begin{table}
        \centering
        \resizebox{\columnwidth}{!}{%
        \begin{tabular}{|c|c|c|c|c|}
        \hline
         Representation & Task & Language & Dataset & Reference \\ 
        \hline
        \hline     
        Bag of Paths & Method name prediction & Java & Java Small/Medium/Large & POPL 2019 \\ \hline 
      %  Graphs       & Variable Naming        & C\#  & MSR ???                 & ICLR 2018 \\ \hline
        Bag of Paths & Method name prediction & Java & Java Small/Medium/Large & ICLR 2019 \\ \hline
        \end{tabular}%
        }
        \caption{Data}
        \label{tab:data}
    \end{table}
\end{comment}


==> results/diff_total/common.tex <==
\begin{table}
    \caption{Change of prediction for all models on all datasets.}
    \label{table:code2vec_js}
    \begin{tabular}{|c|c|c|c|c|c|c|c}
        \hline
        \textbf{Transformation} 
        & \textbf{\#} 
        & \multicolumn{3}{|c|}{\ctv}
        & \multicolumn{3}{|c}{\cts}
        \\ \hline 
         & & 
         \Js & \Jm & \Jl & \Js & \Jm & \Jl
        \\  \hline \hline

        \multirow{4}{*}{\VN} & \#Original programs & 31113 & 235961 & 252725 & 31113 & 235961 & 252725 \\  \cline{2-8}
          & \#Transformed programs & 123123 & 771208 & 916565 & 123123 & 771208 & 916565 \\  \cline{2-8}
          & \#Prediction changing programs & 67622 & 358984 & 385466 & 70371 & 375939 & 431131 \\  \cline{2-8}
          & Prediction change(\%) & 54.92 & 46.55 & 42.06 & 57.16 & 48.75 & 47.04 \\  \hline
        \hline
        
        \multirow{4}{*}{\BX} & \#Original programs & 1158 & 6407 & 8868 & 1158 & 6407 & 8868 \\  \cline{2-8}
          & \#Transformed programs & 1519 & 8840 & 12107 & 1519 & 8840 & 12107 \\  \cline{2-8}
          & \#Prediction changing programs & 818 & 4451 & 5787 & 825 & 3952 & 6227 \\  \cline{2-8}
          & Prediction change(\%) & 53.85 & 50.35 & 47.8 & 54.31 & 44.71 & 51.43 \\  \hline
        \hline
        
        \multirow{4}{*}{\LX} & \#Original programs & 3699 & 17107 & 35565 & 3699 & 17107 & 35565 \\  \cline{2-8}
          & \#Transformed programs & 5160 & 23533 & 49665 & 5160 & 23533 & 49665 \\  \cline{2-8}
          & \#Prediction changing programs & 3064 & 14772 & 23104 & 2711 & 10659 & 21112 \\  \cline{2-8}
          & Prediction change(\%) & 59.38 & 62.77 & 46.52 & 52.54 & 45.29 & 42.51 \\  \hline
        \hline
        
        \multirow{4}{*}{\SF} & \#Original programs & 246 & 3312 & 10478 & 246 & 3312 & 10478 \\  \cline{2-8}
          & \#Transformed programs & 259 & 3839 & 11165 & 259 & 3839 & 11165 \\  \cline{2-8}
          & \#Prediction changing programs & 178 & 2300 & 3386 & 160 & 1597 & 3247 \\  \cline{2-8}
          & Prediction change(\%) & 68.73 & 59.91 & 30.33 & 61.78 & 41.6 & 29.08 \\  \hline
        \hline
        
        \multirow{4}{*}{\PS} & \#Original programs & 15325 & 88865 & 98669 & 15325 & 88865 & 98669 \\  \cline{2-8}
          & \#Transformed programs & 74950 & 366840 & 428263 & 74950 & 366840 & 428263 \\  \cline{2-8}
          & \#Prediction changing programs & 53791 & 232054 & 243574 & 42685 & 170619 & 186411 \\  \cline{2-8}
          & Prediction change(\%) & 71.77 & 63.26 & 56.87 & 56.95 & 46.51 & 43.53 \\  \hline
        \hline
        
        \multirow{4}{*}{\TC} & \#Original programs & 32078 & 232769 & 247092 & 32078 & 232769 & 247092 \\  \cline{2-8}
          & \#Transformed programs & 32078 & 232769 & 247092 & 32078 & 232769 & 247092 \\  \cline{2-8}
          & \#Prediction changing programs & 15039 & 99878 & 88609 & 15490 & 91176 & 87357 \\  \cline{2-8}
          & Prediction change(\%) & 46.88 & 42.91 & 35.86 & 48.29 & 39.17 & 35.35 \\  \hline
        \hline
        
        \multirow{4}{*}{\UN} & \#Original programs & 44426 & 351621 & 370927 & 44426 & 351621 & 370927 \\  \cline{2-8}
          & \#Transformed programs & 44426 & 351621 & 370927 & 44426 & 351621 & 370927 \\  \cline{2-8}
          & \#Prediction changing programs & 17755 & 125880 & 115781 & 20257 & 141511 & 138865 \\  \cline{2-8}
          & Prediction change(\%) & 39.97 & 35.8 & 31.21 & 45.6 & 40.25 & 37.44 \\  \hline
        \hline
        
    \end{tabular}
\end{table}

==> results/scalability_table_new/code2seq.tex <==

\begin{table*}
  \begin{center}
    \caption{\cts (\Jl dataset).}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}|p{2cm}}
            \hline
        \textbf{TS} 
        & \textbf{\#} 
        & \multicolumn{9}{|c|}{Number of Statements in Methods}
        & \textbf{Total} 
        \\ \hline 
        &
        & \textbf{$\leq$ 5} 
        & \textbf{6 $\sim$ 10}
        & \textbf{11  $\sim$ 15}
        & \textbf{16 $\sim$ 20}
        & \textbf{21 $\sim$ 25}
        & \textbf{26 $\sim$ 50}
        & \textbf{51 $\sim$ 100}
        & \textbf{101 $\sim$ 500}
        & \textbf{$\geq$ 501}
        &
        
        \\  \hline \hline

        VN & Original programs & 112536 & 58780 & 29201 & 17080 & 10125 & 18028 & 5433 & 1517 & 25 & 252725 \\  \hline
        VN & Transformed programs & 173347 & 163400 & 123840 & 93767 & 67909 & 166111 & 83940 & 41513 & 2738 & 916565 \\  \hline
        VN & ? programs & [36290, 22087, 62426, 3877, 48667] & [25851, 4317, 77610, 2796, 52826] & [18422, 3116, 54495, 2366, 45441] & [13832, 2291, 36951, 2071, 38622] & [9078, 1642, 25814, 1505, 29870] & [18614, 4814, 57405, 4495, 80783] & [8128, 3182, 25288, 2864, 44478] & [2969, 1532, 11711, 1221, 24080] & [64, 3, 486, 26, 2159] & [133248, 42984, 352186, 21221, 366926] \\  \hline
        VN & ?(\%) & [20.93, 12.74, 36.01, 2.24, 28.07] & [15.82, 2.64, 47.5, 1.71, 32.33] & [14.88, 2.52, 44.0, 1.91, 36.69] & [14.75, 2.44, 39.41, 2.21, 41.19] & [13.37, 2.42, 38.01, 2.22, 43.99] & [11.21, 2.9, 34.56, 2.71, 48.63] & [9.68, 3.79, 30.13, 3.41, 52.99] & [7.15, 3.69, 28.21, 2.94, 58.01] & [2.34, 0.11, 17.75, 0.95, 78.85] & [14.54, 4.69, 38.42, 2.32, 40.03] \\  \hline
        
        BX & Original programs & 450 & 1286 & 1184 & 1025 & 766 & 2192 & 1339 & 612 & 14 & 8868 \\  \hline
        BX & Transformed programs & 474 & 1454 & 1295 & 1141 & 925 & 2811 & 2248 & 1627 & 132 & 12107 \\  \hline
        BX & ? programs & [68, 18, 226, 5, 157] & [217, 49, 613, 70, 505] & [173, 39, 599, 44, 440] & [139, 39, 531, 26, 406] & [90, 23, 373, 23, 416] & [248, 71, 1083, 70, 1339] & [176, 79, 718, 57, 1218] & [116, 35, 487, 55, 934] & [1, 0, 22, 4, 105] & [1228, 353, 4652, 354, 5520] \\  \hline
        BX & ?(\%) & [14.35, 3.8, 47.68, 1.05, 33.12] & [14.92, 3.37, 42.16, 4.81, 34.73] & [13.36, 3.01, 46.25, 3.4, 33.98] & [12.18, 3.42, 46.54, 2.28, 35.58] & [9.73, 2.49, 40.32, 2.49, 44.97] & [8.82, 2.53, 38.53, 2.49, 47.63] & [7.83, 3.51, 31.94, 2.54, 54.18] & [7.13, 2.15, 29.93, 3.38, 57.41] & [0.76, 0.0, 16.67, 3.03, 79.55] & [10.14, 2.92, 38.42, 2.92, 45.59] \\  \hline
        
        LX & Original programs & 994 & 7413 & 6610 & 5311 & 3561 & 7730 & 3009 & 924 & 13 & 35565 \\  \hline
        LX & Transformed programs & 1000 & 7711 & 7539 & 6532 & 4831 & 12219 & 6482 & 3177 & 174 & 49665 \\  \hline
        LX & ? programs & [157, 50, 464, 9, 320] & [1433, 189, 3919, 104, 2066] & [1721, 138, 3378, 115, 2187] & [1782, 135, 2455, 163, 1997] & [1077, 91, 1832, 80, 1751] & [2149, 324, 4200, 350, 5196] & [791, 205, 1985, 208, 3293] & [260, 105, 916, 110, 1786] & [2, 1, 32, 4, 135] & [9372, 1238, 19181, 1143, 18731] \\  \hline
        LX & ?(\%) & [15.7, 5.0, 46.4, 0.9, 32.0] & [18.58, 2.45, 50.82, 1.35, 26.79] & [22.83, 1.83, 44.81, 1.53, 29.01] & [27.28, 2.07, 37.58, 2.5, 30.57] & [22.29, 1.88, 37.92, 1.66, 36.25] & [17.59, 2.65, 34.37, 2.86, 42.52] & [12.2, 3.16, 30.62, 3.21, 50.8] & [8.18, 3.31, 28.83, 3.46, 56.22] & [1.15, 0.57, 18.39, 2.3, 77.59] & [18.87, 2.49, 38.62, 2.3, 37.71] \\  \hline
        
        SF & Original programs & 430 & 1463 & 1758 & 1667 & 1165 & 2570 & 997 & 411 & 17 & 10478 \\  \hline
        SF & Transformed programs & 430 & 1466 & 1774 & 1687 & 1186 & 2662 & 1222 & 699 & 39 & 11165 \\  \hline
        SF & ? programs & [131, 33, 175, 4, 87] & [787, 41, 334, 26, 278] & [1063, 35, 417, 43, 216] & [1218, 18, 160, 23, 268] & [775, 20, 160, 21, 210] & [1311, 207, 415, 102, 627] & [384, 173, 252, 68, 345] & [159, 62, 169, 21, 288] & [4, 1, 4, 5, 25] & [5832, 590, 2086, 313, 2344] \\  \hline
        SF & ?(\%) & [30.47, 7.67, 40.7, 0.93, 20.23] & [53.68, 2.8, 22.78, 1.77, 18.96] & [59.92, 1.97, 23.51, 2.42, 12.18] & [72.2, 1.07, 9.48, 1.36, 15.89] & [65.35, 1.69, 13.49, 1.77, 17.71] & [49.25, 7.78, 15.59, 3.83, 23.55] & [31.42, 14.16, 20.62, 5.56, 28.23] & [22.75, 8.87, 24.18, 3.0, 41.2] & [10.26, 2.56, 10.26, 12.82, 64.1] & [52.23, 5.28, 18.68, 2.8, 20.99] \\  \hline
        
        PS & Original programs & 12797 & 24724 & 17776 & 12604 & 8337 & 15785 & 5222 & 1400 & 24 & 98669 \\  \hline
        PS & Transformed programs & 17635 & 50249 & 48841 & 43655 & 35649 & 109668 & 73743 & 45519 & 3304 & 428263 \\  \hline
        PS & ? programs & [5801, 261, 8640, 230, 2703] & [10539, 555, 29356, 503, 9296] & [7612, 805, 25050, 776, 14598] & [6831, 1160, 19079, 1068, 15517] & [5073, 834, 14769, 807, 14166] & [13022, 2902, 41502, 3809, 48433] & [8717, 2964, 26046, 3191, 32825] & [5173, 2082, 13472, 1557, 23235] & [487, 12, 683, 155, 1967] & [63255, 11575, 178597, 12096, 162740] \\  \hline
        PS & ?(\%) & [32.89, 1.48, 48.99, 1.3, 15.33] & [20.97, 1.1, 58.42, 1.0, 18.5] & [15.59, 1.65, 51.29, 1.59, 29.89] & [15.65, 2.66, 43.7, 2.45, 35.54] & [14.23, 2.34, 41.43, 2.26, 39.74] & [11.87, 2.65, 37.84, 3.47, 44.16] & [11.82, 4.02, 35.32, 4.33, 44.51] & [11.36, 4.57, 29.6, 3.42, 51.04] & [14.74, 0.36, 20.67, 4.69, 59.53] & [14.77, 2.7, 41.7, 2.82, 38.0] \\  \hline
        
        TC & Original programs & 108608 & 62304 & 28476 & 15841 & 9298 & 16331 & 4841 & 1369 & 24 & 247092 \\  \hline
        TC & Transformed programs & 108608 & 62304 & 28476 & 15841 & 9298 & 16331 & 4841 & 1369 & 24 & 247092 \\  \hline
        TC & ? programs & [38124, 4774, 36621, 2349, 26740] & [11697, 1469, 30843, 1079, 17216] & [4607, 637, 13617, 488, 9127] & [2075, 400, 7002, 376, 5988] & [1073, 236, 3871, 215, 3903] & [1622, 476, 6074, 461, 7698] & [435, 182, 1544, 170, 2510] & [97, 50, 424, 46, 752] & [4, 0, 5, 1, 14] & [59734, 8224, 100001, 5185, 73948] \\  \hline
        TC & ?(\%) & [35.1, 4.4, 33.72, 2.16, 24.62] & [18.77, 2.36, 49.5, 1.73, 27.63] & [16.18, 2.24, 47.82, 1.71, 32.05] & [13.1, 2.53, 44.2, 2.37, 37.8] & [11.54, 2.54, 41.63, 2.31, 41.98] & [9.93, 2.91, 37.19, 2.82, 47.14] & [8.99, 3.76, 31.89, 3.51, 51.85] & [7.09, 3.65, 30.97, 3.36, 54.93] & [16.67, 0.0, 20.83, 4.17, 58.33] & [24.17, 3.33, 40.47, 2.1, 29.93] \\  \hline
        
        UN & Original programs & 224048 & 64180 & 30003 & 17316 & 10237 & 18138 & 5455 & 1525 & 25 & 370927 \\  \hline
        UN & Transformed programs & 224048 & 64180 & 30003 & 17316 & 10237 & 18138 & 5455 & 1525 & 25 & 370927 \\  \hline
        UN & ? programs & [72059, 18159, 67643, 4127, 62060] & [12203, 1681, 32312, 821, 17163] & [5442, 670, 13901, 463, 9527] & [3200, 421, 7189, 354, 6152] & [1810, 242, 3990, 216, 3979] & [2810, 611, 6383, 536, 7798] & [815, 214, 1631, 164, 2631] & [208, 59, 455, 43, 760] & [5, 0, 6, 1, 13] & [98552, 22057, 133510, 6725, 110083] \\  \hline
        UN & ?(\%) & [32.16, 8.1, 30.19, 1.84, 27.7] & [19.01, 2.62, 50.35, 1.28, 26.74] & [18.14, 2.23, 46.33, 1.54, 31.75] & [18.48, 2.43, 41.52, 2.04, 35.53] & [17.68, 2.36, 38.98, 2.11, 38.87] & [15.49, 3.37, 35.19, 2.96, 42.99] & [14.94, 3.92, 29.9, 3.01, 48.23] & [13.64, 3.87, 29.84, 2.82, 49.84] & [20.0, 0.0, 24.0, 4.0, 52.0] & [26.57, 5.95, 35.99, 1.81, 29.68] \\  \hline
        \hline
        
    \end{tabular}%
    }
  \end{center}
\end{table*}


==> results/scalability_table_new/readme.tex <==

1. correct prediction stayed as correct prediction
condition: (original == before) & (before == after)
i.e. count,count,count

2. correct prediction swayed into misprediction
condition: (original == before) & (before != after)
i.e. count,count,write

3. incorrect prediction stayed as same incorrect prediction
condition: (original != before) & (before == after)
i.e. count,write,write

4. incorrect prediction remedied into correct prediction
condition: (original != before) & (before != after) & (after == original)
i.e. count,write,count

5. incorrect prediction swayed into different incorrect prediction
condition: (original != before) & (before != after) & (after != original)
i.e. count,write,read


==> results/scalability_table_old/code2seq.tex <==
\begin{table*}
  \begin{center}
    \caption{Change of prediction for \cts on \Js dataset.}
    \label{table:code2seq_js}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
        \hline
        \textbf{Transformation} 
        & \textbf{\#} 
        & \multicolumn{9}{|c|}{Number of Statements in Methods}
        & \textbf{Total} 
        \\ \hline 
        &
        & \textbf{$\leq$ 5} 
        & \textbf{6 $\sim$ 10}
        & \textbf{11  $\sim$ 15}
        & \textbf{16 $\sim$ 20}
        & \textbf{21 $\sim$ 25}
        & \textbf{26 $\sim$ 50}
        & \textbf{51 $\sim$ 100}
        & \textbf{101 $\sim$ 500}
        & \textbf{$\geq$ 501}
        &
        
        \\  \hline \hline

        \multirow{4}{*}{\VN} & Original programs & 11787 & 8122 & 4187 & 2260 & 1418 & 2563 & 680 & 96 & 0 & 31113 \\  \cline{2-12}
          & Transformed programs & 20215 & 22934 & 17895 & 12840 & 9691 & 25228 & 11551 & 2769 & 0 & 123123 \\  \cline{2-12}
          & Prediction changing programs & 9721 & 10329 & 9394 & 7820 & 6197 & 16931 & 8064 & 1915 & 0 & 70371 \\  \cline{2-12}
          & Prediction change(\%) & 48.09 & 45.04 & 52.5 & 60.9 & 63.95 & 67.11 & 69.81 & 69.16 & 0 & 57.16 \\  \hline
        \hline
        
        \multirow{4}{*}{\BX} & Original programs & 32 & 159 & 186 & 140 & 125 & 336 & 147 & 33 & 0 & 1158 \\  \cline{2-12}
          & Transformed programs & 34 & 167 & 199 & 166 & 152 & 452 & 262 & 87 & 0 & 1519 \\  \cline{2-12}
          & Prediction changing programs & 10 & 65 & 72 & 84 & 94 & 271 & 179 & 50 & 0 & 825 \\  \cline{2-12}
          & Prediction change(\%) & 29.41 & 38.92 & 36.18 & 50.6 & 61.84 & 59.96 & 68.32 & 57.47 & 0 & 54.31 \\  \hline
        \hline
        
        \multirow{4}{*}{\LX} & Original programs & 145 & 803 & 675 & 490 & 332 & 880 & 324 & 50 & 0 & 3699 \\  \cline{2-12}
          & Transformed programs & 145 & 828 & 774 & 617 & 471 & 1471 & 691 & 163 & 0 & 5160 \\  \cline{2-12}
          & Prediction changing programs & 43 & 238 & 315 & 313 & 266 & 954 & 467 & 115 & 0 & 2711 \\  \cline{2-12}
          & Prediction change(\%) & 29.66 & 28.74 & 40.7 & 50.73 & 56.48 & 64.85 & 67.58 & 70.55 & 0 & 52.54 \\  \hline
        \hline
        
        \multirow{4}{*}{\SF} & Original programs & 14 & 40 & 43 & 33 & 21 & 57 & 33 & 5 & 0 & 246 \\  \cline{2-12}
          & Transformed programs & 14 & 41 & 45 & 36 & 21 & 61 & 36 & 5 & 0 & 259 \\  \cline{2-12}
          & Prediction changing programs & 6 & 19 & 22 & 23 & 17 & 45 & 25 & 3 & 0 & 160 \\  \cline{2-12}
          & Prediction change(\%) & 42.86 & 46.34 & 48.89 & 63.89 & 80.95 & 73.77 & 69.44 & 60.0 & 0 & 61.78 \\  \hline
        \hline
        
        \multirow{4}{*}{\PS} & Original programs & 1771 & 3933 & 3168 & 1937 & 1294 & 2463 & 666 & 93 & 0 & 15325 \\  \cline{2-12}
          & Transformed programs & 2327 & 7871 & 8903 & 7930 & 6937 & 23971 & 12949 & 4062 & 0 & 74950 \\  \cline{2-12}
          & Prediction changing programs & 577 & 2175 & 3954 & 4364 & 4140 & 15662 & 9039 & 2774 & 0 & 42685 \\  \cline{2-12}
          & Prediction change(\%) & 24.8 & 27.63 & 44.41 & 55.03 & 59.68 & 65.34 & 69.8 & 68.29 & 0 & 56.95 \\  \hline
        \hline
        
        \multirow{4}{*}{\TC} & Original programs & 11750 & 8941 & 4331 & 2288 & 1421 & 2571 & 680 & 96 & 0 & 32078 \\  \cline{2-12}
          & Transformed programs & 11750 & 8941 & 4331 & 2288 & 1421 & 2571 & 680 & 96 & 0 & 32078 \\  \cline{2-12}
          & Prediction changing programs & 5379 & 3678 & 2043 & 1312 & 862 & 1680 & 474 & 62 & 0 & 15490 \\  \cline{2-12}
          & Prediction change(\%) & 45.78 & 41.14 & 47.17 & 57.34 & 60.66 & 65.34 & 69.71 & 64.58 & 0 & 48.29 \\  \hline
        \hline
        
        \multirow{4}{*}{\UN} & Original programs & 23912 & 9047 & 4376 & 2301 & 1434 & 2579 & 681 & 96 & 0 & 44426 \\  \cline{2-12}
          & Transformed programs & 23912 & 9047 & 4376 & 2301 & 1434 & 2579 & 681 & 96 & 0 & 44426 \\  \cline{2-12}
          & Prediction changing programs & 10801 & 3214 & 1961 & 1247 & 856 & 1634 & 477 & 67 & 0 & 20257 \\  \cline{2-12}
          & Prediction change(\%) & 45.17 & 35.53 & 44.81 & 54.19 & 59.69 & 63.36 & 70.04 & 69.79 & 0 & 45.6 \\  \hline
        \hline
        
    \end{tabular}%
    }
  \end{center}
\end{table*}

\begin{table*}
  \begin{center}
    \caption{Change of prediction for \cts on \Jm dataset.}
    \label{table:code2seq_jm}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
        \hline
        \textbf{Transformation} 
        & \textbf{\#} 
        & \multicolumn{9}{|c|}{Number of Statements in Methods}
        & \textbf{Total} 
        \\ \hline 
        &
        & \textbf{$\leq$ 5} 
        & \textbf{6 $\sim$ 10}
        & \textbf{11  $\sim$ 15}
        & \textbf{16 $\sim$ 20}
        & \textbf{21 $\sim$ 25}
        & \textbf{26 $\sim$ 50}
        & \textbf{51 $\sim$ 100}
        & \textbf{101 $\sim$ 500}
        & \textbf{$\geq$ 501}
        &
        
        \\  \hline \hline

        \multirow{4}{*}{\VN} & Original programs & 113756 & 56366 & 25737 & 13728 & 8142 & 14087 & 3540 & 600 & 5 & 235961 \\  \cline{2-12}
          & Transformed programs & 181573 & 159410 & 106993 & 75726 & 53727 & 125360 & 52016 & 16017 & 386 & 771208 \\  \cline{2-12}
          & Prediction changing programs & 82361 & 63048 & 48831 & 38580 & 29047 & 72675 & 31872 & 9389 & 136 & 375939 \\  \cline{2-12}
          & Prediction change(\%) & 45.36 & 39.55 & 45.64 & 50.95 & 54.06 & 57.97 & 61.27 & 58.62 & 35.23 & 48.75 \\  \hline
        \hline
        
        \multirow{4}{*}{\BX} & Original programs & 332 & 1008 & 907 & 839 & 580 & 1723 & 793 & 224 & 1 & 6407 \\  \cline{2-12}
          & Transformed programs & 356 & 1113 & 1045 & 1037 & 721 & 2458 & 1499 & 604 & 7 & 8840 \\  \cline{2-12}
          & Prediction changing programs & 126 & 385 & 345 & 407 & 331 & 1240 & 789 & 325 & 4 & 3952 \\  \cline{2-12}
          & Prediction change(\%) & 35.39 & 34.59 & 33.01 & 39.25 & 45.91 & 50.45 & 52.64 & 53.81 & 57.14 & 44.71 \\  \hline
        \hline
        
        \multirow{4}{*}{\LX} & Original programs & 585 & 3825 & 3337 & 2467 & 1649 & 3726 & 1255 & 262 & 1 & 17107 \\  \cline{2-12}
          & Transformed programs & 587 & 3971 & 3851 & 3145 & 2281 & 6092 & 2730 & 874 & 2 & 23533 \\  \cline{2-12}
          & Prediction changing programs & 187 & 1201 & 1377 & 1374 & 1085 & 3325 & 1575 & 533 & 2 & 10659 \\  \cline{2-12}
          & Prediction change(\%) & 31.86 & 30.24 & 35.76 & 43.69 & 47.57 & 54.58 & 57.69 & 60.98 & 100.0 & 45.29 \\  \hline
        \hline
        
        \multirow{4}{*}{\SF} & Original programs & 302 & 752 & 472 & 417 & 279 & 711 & 289 & 88 & 2 & 3312 \\  \cline{2-12}
          & Transformed programs & 302 & 755 & 482 & 452 & 334 & 924 & 428 & 160 & 2 & 3839 \\  \cline{2-12}
          & Prediction changing programs & 83 & 257 & 166 & 193 & 154 & 473 & 196 & 75 & 0 & 1597 \\  \cline{2-12}
          & Prediction change(\%) & 27.48 & 34.04 & 34.44 & 42.7 & 46.11 & 51.19 & 45.79 & 46.88 & 0.0 & 41.6 \\  \hline
        \hline
        
        \multirow{4}{*}{\PS} & Original programs & 12423 & 24965 & 16759 & 10775 & 6932 & 13004 & 3407 & 595 & 5 & 88865 \\  \cline{2-12}
          & Transformed programs & 17362 & 50585 & 48500 & 41401 & 33509 & 100096 & 54931 & 19968 & 488 & 366840 \\  \cline{2-12}
          & Prediction changing programs & 3329 & 12778 & 18863 & 18778 & 16934 & 56629 & 32651 & 10371 & 286 & 170619 \\  \cline{2-12}
          & Prediction change(\%) & 19.17 & 25.26 & 38.89 & 45.36 & 50.54 & 56.57 & 59.44 & 51.94 & 58.61 & 46.51 \\  \hline
        \hline
        
        \multirow{4}{*}{\TC} & Original programs & 106738 & 60017 & 26101 & 13706 & 8067 & 13999 & 3533 & 601 & 7 & 232769 \\  \cline{2-12}
          & Transformed programs & 106738 & 60017 & 26101 & 13706 & 8067 & 13999 & 3533 & 601 & 7 & 232769 \\  \cline{2-12}
          & Prediction changing programs & 38633 & 21425 & 10447 & 6343 & 4045 & 7828 & 2108 & 346 & 1 & 91176 \\  \cline{2-12}
          & Prediction change(\%) & 36.19 & 35.7 & 40.03 & 46.28 & 50.14 & 55.92 & 59.67 & 57.57 & 14.29 & 39.17 \\  \hline
        \hline
        
        \multirow{4}{*}{\UN} & Original programs & 222841 & 61423 & 26667 & 14011 & 8262 & 14221 & 3580 & 609 & 7 & 351621 \\  \cline{2-12}
          & Transformed programs & 222841 & 61423 & 26667 & 14011 & 8262 & 14221 & 3580 & 609 & 7 & 351621 \\  \cline{2-12}
          & Prediction changing programs & 89443 & 20738 & 10503 & 6425 & 4148 & 7811 & 2090 & 349 & 4 & 141511 \\  \cline{2-12}
          & Prediction change(\%) & 40.14 & 33.76 & 39.39 & 45.86 & 50.21 & 54.93 & 58.38 & 57.31 & 57.14 & 40.25 \\  \hline
        \hline
        
    \end{tabular}%
    }
  \end{center}
\end{table*}

\begin{table*}
  \begin{center}
    \caption{Change in prediction for \cts on \Jl dataset.}
    \label{table:code2seq_jl}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
   
        \hline
        \textbf{Transformation} 
        & \textbf{\#} 
        & \multicolumn{9}{c}{Number of Statements in Methods}
        & \textbf{Total} 
        \\ \hline 
        &
        & \textbf{$\leq$ 5} 
        & \textbf{6 $\sim$ 10}
        & \textbf{11  $\sim$ 15}
        & \textbf{16 $\sim$ 20}
        & \textbf{21 $\sim$ 25}
        & \textbf{26 $\sim$ 50}
        & \textbf{51 $\sim$ 100}
        & \textbf{101 $\sim$ 500}
        & \textbf{$\geq$ 501}
        &
        
        \\  \hline \hline

        \multirow{4}{*}{\VN} & Original programs & 112536 & 58780 & 29201 & 17080 & 10125 & 18028 & 5433 & 1517 & 25 & 252725 \\  \cline{2-12}
          & Transformed programs & 173347 & 163400 & 123840 & 93767 & 67909 & 166111 & 83940 & 41513 & 2738 & 916565 \\  \cline{2-12}
          & Prediction changing programs & 74631 & 59939 & 50923 & 42984 & 33017 & 90092 & 50524 & 26833 & 2188 & 431131 \\  \cline{2-12}
          & Prediction change(\%) & 43.05 & 36.68 & 41.12 & 45.84 & 48.62 & 54.24 & 60.19 & 64.64 & 79.91 & 47.04 \\  \hline
        \hline
        
        \multirow{4}{*}{\BX} & Original programs & 450 & 1286 & 1184 & 1025 & 766 & 2192 & 1339 & 612 & 14 & 8868 \\  \cline{2-12}
          & Transformed programs & 474 & 1454 & 1295 & 1141 & 925 & 2811 & 2248 & 1627 & 132 & 12107 \\  \cline{2-12}
          & Prediction changing programs & 180 & 624 & 523 & 471 & 462 & 1480 & 1354 & 1024 & 109 & 6227 \\  \cline{2-12}
          & Prediction change(\%) & 37.97 & 42.92 & 40.39 & 41.28 & 49.95 & 52.65 & 60.23 & 62.94 & 82.58 & 51.43 \\  \hline
        \hline
        
        \multirow{4}{*}{\LX} & Original programs & 994 & 7413 & 6610 & 5311 & 3561 & 7730 & 3009 & 924 & 13 & 35565 \\  \cline{2-12}
          & Transformed programs & 1000 & 7711 & 7539 & 6532 & 4831 & 12219 & 6482 & 3177 & 174 & 49665 \\  \cline{2-12}
          & Prediction changing programs & 379 & 2359 & 2440 & 2295 & 1922 & 5870 & 3706 & 2001 & 140 & 21112 \\  \cline{2-12}
          & Prediction change(\%) & 37.9 & 30.59 & 32.37 & 35.13 & 39.78 & 48.04 & 57.17 & 62.98 & 80.46 & 42.51 \\  \hline
        \hline
        
        \multirow{4}{*}{\SF} & Original programs & 430 & 1463 & 1758 & 1667 & 1165 & 2570 & 997 & 411 & 17 & 10478 \\  \cline{2-12}
          & Transformed programs & 430 & 1466 & 1774 & 1687 & 1186 & 2662 & 1222 & 699 & 39 & 11165 \\  \cline{2-12}
          & Prediction changing programs & 124 & 345 & 294 & 309 & 251 & 936 & 586 & 371 & 31 & 3247 \\  \cline{2-12}
          & Prediction change(\%) & 28.84 & 23.53 & 16.57 & 18.32 & 21.16 & 35.16 & 47.95 & 53.08 & 79.49 & 29.08 \\  \hline
        \hline
        
        \multirow{4}{*}{\PS} & Original programs & 12797 & 24724 & 17776 & 12604 & 8337 & 15785 & 5222 & 1400 & 24 & 98669 \\  \cline{2-12}
          & Transformed programs & 17635 & 50249 & 48841 & 43655 & 35649 & 109668 & 73743 & 45519 & 3304 & 428263 \\  \cline{2-12}
          & Prediction changing programs & 3194 & 10354 & 16179 & 17745 & 15807 & 55144 & 38980 & 26874 & 2134 & 186411 \\  \cline{2-12}
          & Prediction change(\%) & 18.11 & 20.61 & 33.13 & 40.65 & 44.34 & 50.28 & 52.86 & 59.04 & 64.59 & 43.53 \\  \hline
        \hline
        
        \multirow{4}{*}{\TC} & Original programs & 108608 & 62304 & 28476 & 15841 & 9298 & 16331 & 4841 & 1369 & 24 & 247092 \\  \cline{2-12}
          & Transformed programs & 108608 & 62304 & 28476 & 15841 & 9298 & 16331 & 4841 & 1369 & 24 & 247092 \\  \cline{2-12}
          & Prediction changing programs & 33863 & 19764 & 10252 & 6764 & 4354 & 8635 & 2862 & 848 & 15 & 87357 \\  \cline{2-12}
          & Prediction change(\%) & 31.18 & 31.72 & 36.0 & 42.7 & 46.83 & 52.87 & 59.12 & 61.94 & 62.5 & 35.35 \\  \hline
        \hline
        
        \multirow{4}{*}{\UN} & Original programs & 224048 & 64180 & 30003 & 17316 & 10237 & 18138 & 5455 & 1525 & 25 & 370927 \\  \cline{2-12}
          & Transformed programs & 224048 & 64180 & 30003 & 17316 & 10237 & 18138 & 5455 & 1525 & 25 & 370927 \\  \cline{2-12}
          & Prediction changing programs & 84346 & 19665 & 10660 & 6927 & 4437 & 8945 & 3009 & 862 & 14 & 138865 \\  \cline{2-12}
          & Prediction change(\%) & 37.65 & 30.64 & 35.53 & 40.0 & 43.34 & 49.32 & 55.16 & 56.52 & 56.0 & 37.44 \\  \hline
        \hline
    
    \end{tabular}%
    }
  \end{center}
\end{table*}


==> results/scalability_table_old/code2vec.tex <==
\begin{table*}
    \caption{Change of prediction for \ctv on \Js dataset.}
    \label{table:code2vec_js}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
        \hline
        \textbf{Transformation} 
        & \textbf{\#} 
        & \multicolumn{9}{|Z|}{Number of Statements in Methods}
        & \textbf{Total} 
        \\ \hline 
        &
        & \textbf{$\leq$ 5} 
        & \textbf{6 $\sim$ 10}
        & \textbf{11  $\sim$ 15}
        & \textbf{16 $\sim$ 20}
        & \textbf{21 $\sim$ 25}
        & \textbf{26 $\sim$ 50}
        & \textbf{51 $\sim$ 100}
        & \textbf{101 $\sim$ 500}
        & \textbf{$\geq$ 501}
        &
        
        \\  \hline \hline

        \multirow{4}{*}{\VN} & Original programs & 11787 & 8122 & 4187 & 2260 & 1418 & 2563 & 680 & 96 & 0 & 31113 \\  \cline{2-12}
          & Transformed programs & 20215 & 22934 & 17895 & 12840 & 9691 & 25228 & 11551 & 2769 & 0 & 123123 \\  \cline{2-12}
          & Prediction changing programs & 10627 & 9213 & 7867 & 6746 & 5792 & 17131 & 8517 & 1729 & 0 & 67622 \\  \cline{2-12}
          & Prediction change(\%) & 52.57 & 40.17 & 43.96 & 52.54 & 59.77 & 67.9 & 73.73 & 62.44 & 0 & 54.92 \\  \hline
        \hline
        
        \multirow{4}{*}{\BX} & Original programs & 32 & 159 & 186 & 140 & 125 & 336 & 147 & 33 & 0 & 1158 \\  \cline{2-12}
          & Transformed programs & 34 & 167 & 199 & 166 & 152 & 452 & 262 & 87 & 0 & 1519 \\  \cline{2-12}
          & Prediction changing programs & 12 & 42 & 80 & 72 & 87 & 287 & 185 & 53 & 0 & 818 \\  \cline{2-12}
          & Prediction change(\%) & 35.29 & 25.15 & 40.2 & 43.37 & 57.24 & 63.5 & 70.61 & 60.92 & 0 & 53.85 \\  \hline
        \hline
        
        \multirow{4}{*}{\LX} & Original programs & 145 & 803 & 675 & 490 & 332 & 880 & 324 & 50 & 0 & 3699 \\  \cline{2-12}
          & Transformed programs & 145 & 828 & 774 & 617 & 471 & 1471 & 691 & 163 & 0 & 5160 \\  \cline{2-12}
          & Prediction changing programs & 77 & 367 & 358 & 334 & 269 & 1018 & 518 & 123 & 0 & 3064 \\  \cline{2-12}
          & Prediction change(\%) & 53.1 & 44.32 & 46.25 & 54.13 & 57.11 & 69.2 & 74.96 & 75.46 & 0 & 59.38 \\  \hline
        \hline
        
        \multirow{4}{*}{\SF} & Original programs & 14 & 40 & 43 & 33 & 21 & 57 & 33 & 5 & 0 & 246 \\  \cline{2-12}
          & Transformed programs & 14 & 41 & 45 & 36 & 21 & 61 & 36 & 5 & 0 & 259 \\  \cline{2-12}
          & Prediction changing programs & 7 & 28 & 24 & 20 & 16 & 47 & 32 & 4 & 0 & 178 \\  \cline{2-12}
          & Prediction change(\%) & 50.0 & 68.29 & 53.33 & 55.56 & 76.19 & 77.05 & 88.89 & 80.0 & 0 & 68.73 \\  \hline
        \hline
        
        \multirow{4}{*}{\PS} & Original programs & 1771 & 3933 & 3168 & 1937 & 1294 & 2463 & 666 & 93 & 0 & 15325 \\  \cline{2-12}
          & Transformed programs & 2327 & 7871 & 8903 & 7930 & 6937 & 23971 & 12949 & 4062 & 0 & 74950 \\  \cline{2-12}
          & Prediction changing programs & 613 & 3286 & 5474 & 5626 & 5154 & 19147 & 11090 & 3401 & 0 & 53791 \\  \cline{2-12}
          & Prediction change(\%) & 26.34 & 41.75 & 61.48 & 70.95 & 74.3 & 79.88 & 85.64 & 83.73 & 0 & \textbf{71.77} \\  \hline
        \hline
        
        \multirow{4}{*}{\TC} & Original programs & 11750 & 8941 & 4331 & 2288 & 1421 & 2571 & 680 & 96 & 0 & 32078 \\  \cline{2-12}
          & Transformed programs & 11750 & 8941 & 4331 & 2288 & 1421 & 2571 & 680 & 96 & 0 & 32078 \\  \cline{2-12}
          & Prediction changing programs & 5626 & 3506 & 1763 & 1181 & 786 & 1645 & 479 & 53 & 0 & 15039 \\  \cline{2-12}
          & Prediction change(\%) & 47.88 & 39.21 & 40.71 & 51.62 & 55.31 & 63.98 & 70.44 & 55.21 & 0 & 46.88 \\  \hline
        \hline
        
        \multirow{4}{*}{\UN} & Original programs & 23912 & 9047 & 4376 & 2301 & 1434 & 2579 & 681 & 96 & 0 & 44426 \\  \cline{2-12}
          & Transformed programs & 23912 & 9047 & 4376 & 2301 & 1434 & 2579 & 681 & 96 & 0 & 44426 \\  \cline{2-12}
          & Prediction changing programs & 9948 & 2338 & 1485 & 1041 & 773 & 1632 & 473 & 65 & 0 & 17755 \\  \cline{2-12}
          & Prediction change(\%) & 41.6 & 25.84 & 33.94 & 45.24 & 53.91 & 63.28 & 69.46 & 67.71 & 0 & 39.97 \\  \hline
        \hline
        
    \end{tabular}%
   }
\end{table*}

\begin{table*}
  \begin{center}
    \caption{Change of prediction for \ctv on \Jm dataset.}
    \label{table:code2vec_jm}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
        \hline
        \textbf{Transformation} 
        & \textbf{\#} 
        & \multicolumn{9}{|c|}{Number of Statements in Methods}
        & \textbf{Total} 
        \\ \hline 
        &
        & \textbf{$\leq$ 5} 
        & \textbf{6 $\sim$ 10}
        & \textbf{11  $\sim$ 15}
        & \textbf{16 $\sim$ 20}
        & \textbf{21 $\sim$ 25}
        & \textbf{26 $\sim$ 50}
        & \textbf{51 $\sim$ 100}
        & \textbf{101 $\sim$ 500}
        & \textbf{$\geq$ 501}
        &
        
        \\  \hline \hline

        \multirow{4}{*}{\VN} & Original programs & 113756 & 56366 & 25737 & 13728 & 8142 & 14087 & 3540 & 600 & 5 & 235961 \\  \cline{2-12}
          & Transformed programs & 181573 & 159410 & 106993 & 75726 & 53727 & 125360 & 52016 & 16017 & 386 & 771208 \\  \cline{2-12}
          & Prediction changing programs & 85053 & 47411 & 37655 & 33718 & 28045 & 77540 & 37020 & 12462 & 80 & 358984 \\  \cline{2-12}
          & Prediction change(\%) & 46.84 & 29.74 & 35.19 & 44.53 & 52.2 & 61.85 & 71.17 & 77.8 & 20.73 & 46.55 \\  \hline
        \hline
        
        \multirow{4}{*}{\BX} & Original programs & 332 & 1008 & 907 & 839 & 580 & 1723 & 793 & 224 & 1 & 6407 \\  \cline{2-12}
          & Transformed programs & 356 & 1113 & 1045 & 1037 & 721 & 2458 & 1499 & 604 & 7 & 8840 \\  \cline{2-12}
          & Prediction changing programs & 158 & 352 & 316 & 389 & 354 & 1426 & 1001 & 451 & 4 & 4451 \\  \cline{2-12}
          & Prediction change(\%) & 44.38 & 31.63 & 30.24 & 37.51 & 49.1 & 58.01 & 66.78 & 74.67 & 57.14 & 50.35 \\  \hline
        \hline
        
        \multirow{4}{*}{\LX} & Original programs & 585 & 3825 & 3337 & 2467 & 1649 & 3726 & 1255 & 262 & 1 & 17107 \\  \cline{2-12}
          & Transformed programs & 587 & 3971 & 3851 & 3145 & 2281 & 6092 & 2730 & 874 & 2 & 23533 \\  \cline{2-12}
          & Prediction changing programs & 410 & 2398 & 2036 & 1703 & 1380 & 4110 & 2018 & 717 & 0 & 14772 \\  \cline{2-12}
          & Prediction change(\%) & 69.85 & 60.39 & 52.87 & 54.15 & 60.5 & 67.47 & 73.92 & 82.04 & 0.0 & 62.77 \\  \hline
        \hline
        
        \multirow{4}{*}{\SF} & Original programs & 302 & 752 & 472 & 417 & 279 & 711 & 289 & 88 & 2 & 3312 \\  \cline{2-12}
          & Transformed programs & 302 & 755 & 482 & 452 & 334 & 924 & 428 & 160 & 2 & 3839 \\  \cline{2-12}
          & Prediction changing programs & 141 & 418 & 270 & 248 & 193 & 589 & 312 & 128 & 1 & 2300 \\  \cline{2-12}
          & Prediction change(\%) & 46.69 & 55.36 & 56.02 & 54.87 & 57.78 & 63.74 & 72.9 & 80.0 & 50.0 & 59.91 \\  \hline
        \hline
        
        \multirow{4}{*}{\PS} & Original programs & 12423 & 24965 & 16759 & 10775 & 6932 & 13004 & 3407 & 595 & 5 & 88865 \\  \cline{2-12}
          & Transformed programs & 17362 & 50585 & 48500 & 41401 & 33509 & 100096 & 54931 & 19968 & 488 & 366840 \\  \cline{2-12}
          & Prediction changing programs & 4240 & 16739 & 23414 & 24078 & 22132 & 75718 & 46926 & 18319 & 488 & 232054 \\  \cline{2-12}
          & Prediction change(\%) & 24.42 & 33.09 & 48.28 & 58.16 & 66.05 & 75.65 & 85.43 & 91.74 & 100.0 & \textbf{63.26} \\  \hline
        \hline
        
        \multirow{4}{*}{\TC} & Original programs & 106738 & 60017 & 26101 & 13706 & 8067 & 13999 & 3533 & 601 & 7 & 232769 \\  \cline{2-12}
          & Transformed programs & 106738 & 60017 & 26101 & 13706 & 8067 & 13999 & 3533 & 601 & 7 & 232769 \\  \cline{2-12}
          & Prediction changing programs & 44808 & 22821 & 10167 & 6322 & 4264 & 8549 & 2474 & 470 & 3 & 99878 \\  \cline{2-12}
          & Prediction change(\%) & 41.98 & 38.02 & 38.95 & 46.13 & 52.86 & 61.07 & 70.03 & 78.2 & 42.86 & 42.91 \\  \hline
        \hline
        
        \multirow{4}{*}{\UN} & Original programs & 222841 & 61423 & 26667 & 14011 & 8262 & 14221 & 3580 & 609 & 7 & 351621 \\  \cline{2-12}
          & Transformed programs & 222841 & 61423 & 26667 & 14011 & 8262 & 14221 & 3580 & 609 & 7 & 351621 \\  \cline{2-12}
          & Prediction changing programs & 83704 & 13957 & 7927 & 5440 & 3923 & 8070 & 2400 & 456 & 3 & 125880 \\  \cline{2-12}
          & Prediction change(\%) & 37.56 & 22.72 & 29.73 & 38.83 & 47.48 & 56.75 & 67.04 & 74.88 & 42.86 & 35.8 \\  \hline
        \hline
        
    \end{tabular}%
    }
  \end{center}
\end{table*}

\begin{table*}
  \begin{center}
    \caption{Change of prediction for \ctv on \Jl dataset.}
    \label{table:code2vec_jl}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
        \hline
        \textbf{Transformation} 
        & \textbf{\#} 
        & \multicolumn{9}{|c|}{Number of Statements in Methods}
        & \textbf{Total} 
        \\ \hline 
        &
        & \textbf{$\leq$ 5} 
        & \textbf{6 $\sim$ 10}
        & \textbf{11  $\sim$ 15}
        & \textbf{16 $\sim$ 20}
        & \textbf{21 $\sim$ 25}
        & \textbf{26 $\sim$ 50}
        & \textbf{51 $\sim$ 100}
        & \textbf{101 $\sim$ 500}
        & \textbf{$\geq$ 501}
        &
        
        \\  \hline \hline
        
        \multirow{4}{*}{\VN} & Original programs & 112536 & 58780 & 29201 & 17080 & 10125 & 18028 & 5433 & 1517 & 25 & 252725 \\  \cline{2-12}
          & Transformed programs & 173347 & 163400 & 123840 & 93767 & 67909 & 166111 & 83940 & 41513 & 2738 & 916565 \\  \cline{2-12}
          & Prediction changing programs & 66968 & 39543 & 35841 & 34680 & 30580 & 92082 & 55941 & 28713 & 1118 & 385466 \\  \cline{2-12}
          & Prediction change(\%) & 38.63 & 24.2 & 28.94 & 36.99 & 45.03 & 55.43 & 66.64 & 69.17 & 40.83 & 42.06 \\  \hline
        \hline
        
        \multirow{4}{*}{\BX} & Original programs & 450 & 1286 & 1184 & 1025 & 766 & 2192 & 1339 & 612 & 14 & 8868 \\  \cline{2-12}
          & Transformed programs & 474 & 1454 & 1295 & 1141 & 925 & 2811 & 2248 & 1627 & 132 & 12107 \\  \cline{2-12}
          & Prediction changing programs & 159 & 382 & 367 & 350 & 374 & 1464 & 1494 & 1129 & 68 & 5787 \\  \cline{2-12}
          & Prediction change(\%) & 33.54 & 26.27 & 28.34 & 30.67 & 40.43 & 52.08 & 66.46 & 69.39 & 51.52 & 47.8 \\  \hline
        \hline
        
        \multirow{4}{*}{\LX} & Original programs & 994 & 7413 & 6610 & 5311 & 3561 & 7730 & 3009 & 924 & 13 & 35565 \\  \cline{2-12}
          & Transformed programs & 1000 & 7711 & 7539 & 6532 & 4831 & 12219 & 6482 & 3177 & 174 & 49665 \\  \cline{2-12}
          & Prediction changing programs & 479 & 3009 & 2340 & 2274 & 2022 & 6575 & 4245 & 2095 & 65 & 23104 \\  \cline{2-12}
          & Prediction change(\%) & 47.9 & 39.02 & 31.04 & 34.81 & 41.85 & 53.81 & 65.49 & 65.94 & 37.36 & 46.52 \\  \hline
        \hline
        
        \multirow{4}{*}{\SF} & Original programs & 430 & 1463 & 1758 & 1667 & 1165 & 2570 & 997 & 411 & 17 & 10478 \\  \cline{2-12}
          & Transformed programs & 430 & 1466 & 1774 & 1687 & 1186 & 2662 & 1222 & 699 & 39 & 11165 \\  \cline{2-12}
          & Prediction changing programs & 148 & 320 & 267 & 246 & 289 & 1055 & 602 & 433 & 26 & 3386 \\  \cline{2-12}
          & Prediction change(\%) & 34.42 & 21.83 & 15.05 & 14.58 & 24.37 & 39.63 & 49.26 & 61.95 & 66.67 & 30.33 \\  \hline
        \hline
        
        \multirow{4}{*}{\PS} & Original programs & 12797 & 24724 & 17776 & 12604 & 8337 & 15785 & 5222 & 1400 & 24 & 98669 \\  \cline{2-12}
          & Transformed programs & 17635 & 50249 & 48841 & 43655 & 35649 & 109668 & 73743 & 45519 & 3304 & 428263 \\  \cline{2-12}
          & Prediction changing programs & 2451 & 10904 & 17892 & 20813 & 19591 & 73100 & 55791 & 39814 & 3218 & 243574 \\  \cline{2-12}
          & Prediction change(\%) & 13.9 & 21.7 & 36.63 & 47.68 & 54.96 & 66.66 & 75.66 & 87.47 & 97.4 & \textbf{56.87} \\  \hline
        \hline
        
        \multirow{4}{*}{\TC} & Original programs & 108608 & 62304 & 28476 & 15841 & 9298 & 16331 & 4841 & 1369 & 24 & 247092 \\  \cline{2-12}
          & Transformed programs & 108608 & 62304 & 28476 & 15841 & 9298 & 16331 & 4841 & 1369 & 24 & 247092 \\  \cline{2-12}
          & Prediction changing programs & 37841 & 18628 & 8973 & 6108 & 4222 & 8792 & 3094 & 940 & 11 & 88609 \\  \cline{2-12}
          & Prediction change(\%) & 34.84 & 29.9 & 31.51 & 38.56 & 45.41 & 53.84 & 63.91 & 68.66 & 45.83 & 35.86 \\  \hline
        \hline
        
        \multirow{4}{*}{\UN} & Original programs & 224048 & 64180 & 30003 & 17316 & 10237 & 18138 & 5455 & 1525 & 25 & 370927 \\  \cline{2-12}
          & Transformed programs & 224048 & 64180 & 30003 & 17316 & 10237 & 18138 & 5455 & 1525 & 25 & 370927 \\  \cline{2-12}
          & Prediction changing programs & 76338 & 10658 & 6472 & 5237 & 3911 & 8919 & 3272 & 965 & 9 & 115781 \\  \cline{2-12}
          & Prediction change(\%) & 34.07 & 16.61 & 21.57 & 30.24 & 38.2 & 49.17 & 59.98 & 63.28 & 36.0 & 31.21 \\  \hline
        \hline
        
    \end{tabular}%
    }
  \end{center}
\end{table*}


==> robustness.tex <==
\section{Robustness of NN Models for Code}
In this section, we formalize the notion of robustness of models of code. 

==> texstufftemp.tex <==
\usepackage[ textsize=tiny, textwidth=1.4cm]{todonotes}

\newcommand{\Amin}[1]{\todo[color=red!10, linecolor=black!30!red!50!white]{\textbf{Fix}: #1}}

\newcommand{\TODO}[1]{\todo[color=red!10, linecolor=black!30!red!50!white]{\textbf{TODO}: #1}}


\newcommand{\Fix}[1]{\textbf{Fix:#1}}
\newcommand{\Space}[1]{}

\newcommand{\Etal}{\emph{et al.}}
\newcommand{\Eg}{\emph{}{e.g.}}
\newcommand{\Ie}{\emph{}{i.e.}}
\newcommand{\Viz}{\emph{viz.}}
\newcommand{\Insitu}{\emph{in situ}}

\newcommand{\Aka}{\emph{aka}}
\usepackage{xspace}
\newcommand{\SO}{Stack Overflow\xspace}

\newcommand{\Comment}[1]{}
\newcounter{observation}
\newcommand{\observation}[1]{\refstepcounter{observation}
        \begin{center}
        \Ovalbox{
        \begin{minipage}{0.93\columnwidth}
                \textbf{Observation \arabic{observation}:} #1
        \end{minipage}
        }
        \end{center}
        \vspace{-5pt}
}

==> transformation-example/all.tex <==
\subsection{Example of Transformation}
\input{transformation-example/variable-renaming.tex}
\input{transformation-example/loop-exchange.tex}
\input{transformation-example/switch-to-if.tex}
\input{transformation-example/boolean-exchange.tex}
\input{transformation-example/permute-stmt.tex}
\input{transformation-example/trycatch-insertion.tex}
\input{transformation-example/unused-stmt-insertion.tex}


==> transformation-example/boolean-exchange.tex <==
\subsubsection{Boolean Exchange}
Given a method $M$, visit the AST and locate the boolean nodes into a list, $boolList$. For each boolean node $bool_{i} \; \epsilon \; boolList$, change the $true$ with $false$ (and vice versa) and neglect the condition of $bool_{i}$ in $M$ to keep the semantic.

$\newline$
Before:
$\newline$
\begin{lstlisting}
    void flagDemo() {
            boolean flag = true;
            if (flag) {
                    System.out.println("True Condition");
            } else {
                    System.out.println("False Condition");
            }
    }
\end{lstlisting}

$\newline$
After:
\begin{lstlisting}
    void flagDemo() {
        boolean flag = false;
        if (!flag) {
            System.out.println("True Condition");
        } else {
            System.out.println("False Condition");
        }
    }
\end{lstlisting}



==> transformation-example/loop-exchange.tex <==
\subsubsection{Loop Exchange}
Given a method $M$, visit the AST and locate the loop nodes ($for$ and $while$) into a list, $loopList$. For each loop node $loop_{i} \; \epsilon \; loopList$, replace the $for$ node by creating a $while$ node, and vice versa.

$\newline$
Before:
$\newline$
\begin{lstlisting}
    boolean isPrime(int n) {
        if (n <= 1) {
            return false;
        }
        for (int i = 2; i < Math.sqrt(n); i++) {
            if (n % i == 0) {
                return false;
            }
        }
        return true;
    }
\end{lstlisting}

$\newline$
After:
\begin{lstlisting}
    boolean isPrime(int n) {
        if (n <= 1) {
            return false;
        }
        {
            int i = 2;
            while (i < Math.sqrt(n)) {
                if (n % i == 0) {
                    return false;
                }
                i++;
            }
        }
        return true;
    }
\end{lstlisting}


==> transformation-example/permute-stmt.tex <==
\subsubsection{Permute Statement}
Given a method $M$, visit the AST and locate the statement nodes into a list, $stmtList$. For each pair of statements $stmt_{i} \; \epsilon \; stmtList$ and $stmt_{j} \; \epsilon \; stmtList$, swap $stmt_{i}$ with $stmt_{j}$ in $M$ if there is no dependency among them.

$\newline$
Before:
$\newline$
\begin{lstlisting}
    void addTwoValues() {
        int value1 = 10;
        int value2 = 20;
        int sum = value1 + value2;
        System.out.println("Sum = " + sum);
    }
\end{lstlisting}

$\newline$
After:
\begin{lstlisting}
    void addTwoValues() {
        int value2 = 20;
        int value1 = 10;
        int sum = value1 + value2;
        System.out.println("Sum = " + sum);
    }
\end{lstlisting}

==> transformation-example/switch-to-if.tex <==
\subsubsection{Switch to If}
Given a method $M$, visit the AST and locate the switch nodes into a list, $switchList$. For each switch node $switch_{i} \; \epsilon \; switchList$, replace it in $M$ by creating a $if-else$ node.

$\newline$
Before:
$\newline$
\begin{lstlisting}
    void simpleCalculation(int n1, int n2, char op){
        int result = 0;
        switch (op) {
            case '+':
                result = n1 + n2;
                break;
            case '-':
                result = n1 - n2;
                break;
            case '*':
                result = n1 * n2;
                break;
            case '/':
                result = n1 / n2;
                break;
            default:
                System.out.println("Unknown op!");
                break;
        }
        System.out.print(n1 + " " + op + " " + n2 + " = " + result);
    }
\end{lstlisting}

$\newline$
After:
\begin{lstlisting}
    void simpleCalculation(int n1, int n2, char op) {
        int result = 0;
        if (op == '+') {
            result = n1 + n2;
        } else if (op == '-') {
            result = n1 - n2;
        } else if (op == '*') {
            result = n1 * n2;
        } else if (op == '/') {
            result = n1 / n2;
        } else {
            System.out.println("Unknown op!");
        }
        System.out.print(n1 + " " + op + " " + n2 + " = " + result);
    }
\end{lstlisting}

==> transformation-example/trycatch-insertion.tex <==
\subsubsection{Try Catch Insertion}
Given a method $M$, visit the AST and surround a randomly selected \textit{non-declarative expression} statement by a \textit{try catch} block.

$\newline$
Before:
$\newline$
\begin{lstlisting}
    void addTwoValues() {
        int value1 = 10;
        int value2 = 20;
        int sum = value1 + value2;
        System.out.println("Sum = " + sum);
    }
\end{lstlisting}

$\newline$
After:
\begin{lstlisting}
    void addTwoValues() {
        try {
            int value1 = 10;
            int value2 = 20;
            int sum = value1 + value2;
            System.out.println("Sum = " + sum);
        } catch (Exception ex) {
            ex.printStackTrace();
        }
    }
\end{lstlisting}

==> transformation-example/unreachable-stmt-insertion.tex <==
\subsubsection{Unreachable Statement Insertion}
Given a method $M$, visit the AST and insert an \textit{if} block of \textit{false} condition at random place of $M$ such that the body of \textit{if} is unreachable.

$\newline$
Before:
$\newline$
\begin{lstlisting}
    void addTwoValues() {
        int value1 = 10;
        int value2 = 20;
        int sum = value1 + value2;
        System.out.println("Sum = " + sum);
    }
\end{lstlisting}

$\newline$
After:
\begin{lstlisting}
    void addTwoValues() {
        int value1 = 10;
        int value2 = 20;
        if (false) {
            System.out.println("an unreachable statement");
        }
        int sum = value1 + value2;
        System.out.println("Sum = " + sum);
    }
\end{lstlisting}

==> transformation-example/unused-stmt-insertion.tex <==
\subsubsection{Unused Statement Insertion}
Given a method $M$, visit the AST and insert a \textit{string declaration} (initialized with \textit{timestamp}) at random place of $M$ such that the \textit{string} is never used.

$\newline$
Before:
$\newline$
\begin{lstlisting}
    void addTwoValues() {
        int value1 = 10;
        int value2 = 20;
        int sum = value1 + value2;
        System.out.println("Sum = " + sum);
    }
\end{lstlisting}

$\newline$
After:
\begin{lstlisting}
    void addTwoValues() {
        int value1 = 10;
        int value2 = 20;
        int sum = value1 + value2;
        String dummy_timestamp = "2019-12-16 13:41:48.916";
        System.out.println("Sum = " + sum);
    }
\end{lstlisting}

==> transformation-example/variable-renaming.tex <==
\subsubsection{Variable Renaming}
Given a method $M$, visit the AST and locate the nodes into a list, $varList$. For each variable node $v_{i} \; \epsilon \; varList$, change the name of $v_{i}$ in $M$ by $var_{i}$.

$\newline$
Before:
$\newline$
\begin{lstlisting}
    void printArray(int arr[]) {
        for (int i = 0; i < arr.length; ++i) {
            System.out.print(arr[i] + " ");
        }
    }
\end{lstlisting}

$\newline$
After:
\begin{lstlisting}
    void printArray(int[] var0) {
        for (int var1 = 0; var1 < var0.length; ++var1) {
            System.out.print(var0[var1] + " ");
        }
    }
\end{lstlisting}
